Bridging Quantum Computing and Differential Privacy: Insights into Quantum Computing Privacy

While quantum computing has strong potential in data-driven fields, the privacy issue of sensitive or valuable information involved in the quantum algorithm should be considered. Differential privacy (DP), which is a fundamental privacy tool widely used in the classical scenario, has been extended to the quantum domain, i.e., quantum differential privacy (QDP). QDP may become one of the most promising approaches toward privacy-preserving quantum computing since it is not only compatible with classical DP mechanisms but also achieves privacy protection by exploiting unavoidable quantum noise in noisy intermediate-scale quantum (NISQ) devices. This paper provides an overview of the various implementations of QDP and their performance in terms of privacy parameters under the DP setting. Specifically, we propose a taxonomy of QDP techniques, categorizing the literature on whether internal or external randomization is used as a source to achieve QDP and how these implementations are applied to each phase of the quantum algorithm. We also discuss challenges and future directions for QDP. By summarizing recent advancements, we hope to provide a comprehensive, up-to-date review for researchers venturing into this field.

==> contents/0.abstract.tex <==
\begin{abstract}

While quantum computing has a strong potential in data-driven fields, privacy and security issues on sensitive or valuable information that involved in the quantum algorithm should be concerned. As differential privacy (DP), which is a fundamental privacy tool widely used in the classical scenario, has been extended to the quantum domain. Quantum differential privacy (QDP) may become one of the most promising avenues for privacy-preserving quantum algorithms, since it is not only compatible with the classical mechanisms of DP, but also achieves DP by exploiting unavoidable quantum noise in NISQ devices as a privacy element. This paper provides an overview of the various implementation approaches of QDP and their performance of privacy parameters under the DP setting. Concretely speaking, we categorize the existing literature based on whether whether internal or external randomization is used as a source to achieve QDP and explore how these approaches are applied on phases of the quantum algorithm. We also discuss challenges and future directions for DP in quantum computing. By summarizing recent advancements, we hope to provide a comprehensive, up-to-date overview for researchers venturing into this field.
\end{abstract}

%In this survey, we categorize the existing literature based on whether internal inherent noise or external artificial noise is used as a source to achieve DP in quantum computing. We explore how these approaches are applied at different stages of a quantum algorithm (i.e., state preparation, quantum circuit, and quantum measurement). We also discuss challenges and future directions for DP in quantum computing. By summarizing recent advancements, we hope to provide a comprehensive, up-to-date overview for researchers venturing into this field.

==> contents/table.tex <==
    \vspace{-1pt}
    \begin{wraptable}{r}{0.5\textwidth}
        \footnotesize
        \centering
        \caption{Summary of notations}
        \label{tab:notation}
        \scriptsize
        \begin{tabular}{c|c}
            \toprule                
            Symbol & Definition  \\
            \midrule
            $\mathcal{A}$ & a quantum algorithm \\
            $\mathcal{I}$ & input of quantum algorithm \\
            $\mathcal{O}$ & output of quantum algorithm \\
            $\mathcal{H}$ & Hilbert space \\
            $\mathcal{D}$ & domain of classical data \\
            $\mathcal{E}$ & quantum channel (super-operator) \\
            $\mathcal{E}^\dagger$ & dual form of quantum channel $\mathcal{E}$\\
            $\mathcal{N}$ & noise model \\
            $\mathbb{I}$ & identity matrix \\
            $N$ & the number of qubits \\
            $K$ & quantum minimum adjacent kernel\\
            $n_{\mathrm{shot}}$ & the number of shots \\
            $x$ & data point (vector) from classical dataset \\
            $|i\rangle$ & a set of orthonormal basis in Hilbert space \\
            $|\rho \rangle, |\sigma\rangle$ & pure quantum state \\
            $\rho, \sigma$ & mixed quantum state \\
            $D$ & dimension of Hilbert space $\mathcal{H}$ \\
            $U$ & quantum gate \\
            $M$ & a set of measurements \\
            $E$ & a Kraus operator \\
            $\tau(\cdot,\cdot)$ & distance metric between states \\
            $\mathrm{Tr}(\cdot)$ & trace of a matrix\\
            $\epsilon$ & privacy budget \\
            $\delta$ & fault tolerance rate\\  
            $p$ & probability of gate flipping in Pauli channels \\
            $\alpha$ & factor of hockey-stick divergence\\
            $\beta$ & upper bound of contraction coefficient\\
            $\gamma$ & error probability of amplitude damping channel \\
            $\lambda$ & error probability of phase damping channel \\
            \bottomrule
        \end{tabular}
    \end{wraptable}
    \vspace{-1pt}
